Robust Optimal Network Topology Switching for Zero Dynamics Attacks

The intrinsic, sampling, and enforced zero dynamics attacks (ZDAs) are among the most detrimental stealthy attacks in robotics, aerospace, and cyber-physical systems. They exploit internal dynamics, discretization, redundancy/asynchronous actuation and sensing, to construct disruptive attacks that are completely stealthy in the measurement. They work even when the systems are both controllable and observable. This paper presents a novel framework to robustly and optimally detect and mitigate ZDAs for networked linear control systems. We utilize controllability, observability, robustness, and sensitivity metrics written explicitly in terms of the system topology, thereby proposing a robust and optimal switching topology formulation for resilient ZDA detection and mitigation. Our main contribution is the reformulation of this problem into an equivalent rank-constrained optimization problem (i.e., optimization with a convex objective function subject to convex constraints and rank constraints), which can be solved using convex rank minimization approaches. The effectiveness of our method is demonstrated using networked double integrators subject to ZDAs.

==> sections/archived_sections/1_abstract.tex <==
\begin{abstract}
\htred{authors \& their order TBD}{}
The intrinsic, sampling, and enforced zero dynamics attacks (ZDAs) are among the most lethal but common stealthy attacks in robotics, aerospace, and cyber-physical systems. They exploit internal dynamics, discretization, or actuation redundancy/asynchronous actuation and sensing, respectively, to construct disruptive attacks completely stealthy in the system measurement. Surprisingly, they work even when the systems are both controllable and observable. This paper thus presents a novel framework to robustly and optimally detect ZDAs for networked linear control systems. We define controllability, observability, robustness, and sensitivity metrics, written explicitly in terms of the system topology, thereby proposing a robust and optimal topology switching problem for resilient ZDA detection. \TBD{This problem is solved using a sequential convex approach, utilizing the unique structure of the system}. Our approach is demonstrated in several networked dynamical systems subject to ZDAs.
\end{abstract}
%\begin{keywords}
%Robust control, Autonomous systems, and Machine learning.
%\end{keywords}
% Our main contribution is to enhance the performance of the learned motion planning policy with collision avoidance and tracking-based robustness guarantees, independently of its original performance such as approximation errors and regret bounds in machine learning.

==> sections/archived_sections/2_introduction.tex <==
\section{Introduction}
\label{sec_introduction}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\begin{itemize}
    \item show convexity at least for $B$ and $C$?
    \item remark on $\Phi_k$ (fault state)
    \item justify discrete actuation and sensing
    \item sensor attack -> future work unfortunately
    \item note on robust ZDA/nonlinear ZDA in the introduction (for uncertain systems or nonlinear systems, there exists a robust version of ZDAs~\cite{robust_zda})
    \item emphasize that our approach is different from~\cite{zda_continuous_hovakimyan,uavzda,zda_discrete} in that it is 1) robust and optimal 2) it is more general considering enforced ZDA
    \item Guarantee synchronization even with switching?
    \item connection to flexible structure for the topology-dependent B matrix
    \item relationship btw zda and network properties
    \item make sure we cite~\cite{security_metric_book} when we talk about security metrics and convex formulation
    \item Also, we could consider other metrics, especially the output-to-output gain~\cite{security_metric_book} to generalize the metric based on $\mathcal{H}_{\infty}$ and $\mathcal{H}_{-}$ with more useful properties.
    \begin{itemize}
        \item But this metric requires solving a convex optimization just to compute a metric for a given topology which requires additional computation
        \item Also, when $C_k$ is a decision variable, then the constraint of the output-to-output gain is no longer LMI or BMI
    \end{itemize}
    \item some other attacks left for future work
    \item form of detectors (like residual detectors): future work
    \item invariant zeros are invariant under feedback
    \item causal systems -> invertible
    \item Adding estimation gets messy, let's just cite~\cite{outputL2gain} to use $u = -Kx+\bar{u}$ and put a remark on state estimation \eg{},~$u = [0,-K][x^{\top},\hat{x}^{\top}]^{\top}$
\end{itemize}
\subsubsection*{Contributions}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsubsection*{Related Work}

%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsubsection*{Notation}
%For $A \in \mathbb{R}^{n \times n}$, we use $A \succ 0$, $A \succeq 0$, $A \prec 0$, and $A \preceq 0$ for the positive definite, positive semi-definite, negative definite, negative semi-definite matrices, respectively. For $x \in \mathbb{R}^n$ and $A \in \mathbb{R}^{n \times m}$, we let $\|x\|$, $\|x\|_{\Xi}$, $\|A\|$, $\|A\|_F$ denote the Euclidean norm, weighted $2$-norm (\ie{}, $\|x\|_{\Xi}=\sqrt{x^{\top}\Xi x}$ for $\Xi \succ 0$), induced 2-norm, and Frobenius norm, respectively. Also, $\mathop{\mathbb{E}}$ denotes the expected value operator.
%, and $\sym(A) = (A+A^{\top})/2$
\label{notation}


==> sections/archived_sections/3_preliminaries.tex <==
\section{Preliminaries and Problem Statement}
\label{sec_preliminaries}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
In this paper, we consider the following continuous-time, networked linear control system:
\begin{align}
    \dot{x}(t) &= A(\nu(t)) x(t)+B_u(\nu(t))u(y(t),\nu(t))+B_a(\nu(t))a(t)\label{eq_continuous_initialx}\\
    y(t) &= C(\nu(t))x(t)+D(\nu(t))a(t)\label{eq_continuous_initialy}
\end{align}
where $t \in \mathbb{R}_{+}$, $\nu:\mathbb{R}_{+}\mapsto\mathcal{T}$ is the topology representation of the network (\eg{}, adjacency matrix) with $\mathcal{T}$ being the set of topologies, $x:\mathbb{R}_{+}\mapsto\mathbb{R}^p$ is the stacked system state, $u:\mathbb{R}_{+}\mapsto\mathbb{R}^q$ is the stacked system control input, $a:\mathbb{R}_{+}\mapsto\mathbb{R}^r$ is the stacked attack control input, $y:\mathbb{R}_{+}\mapsto\mathbb{R}^s$ is the stacked system measurement, and $A:\mathcal{T}\mapsto\mathbb{R}^{p\times p}$, $B_u:\mathcal{T}\mapsto\mathbb{R}^{p\times q}$, $B_a:\mathcal{T}\mapsto\mathbb{R}^{p\times r}$, and $C:\mathcal{T}\mapsto\mathbb{R}^{s\times p}$, and $D:\mathcal{T}\mapsto\mathbb{R}^{s\times r}$ the stacked system matrices.
\begin{remark}
\label{remark_estimation}
This formulation can be viewed as a general closed-loop dynamical system, where $x$ consists of the actual state, estimated state for feedback control, and estimated state for anomaly detection as in~\cite{outputL2gain}.
\end{remark}
\begin{assumption}
\label{assump_system}
We assume the following in~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy}:
\begin{enumerate}[label={\color{uiucblue}{\rm(\alph*)}}]
    \item The functions $A$, $B_u$, $B_a$, $C$, and $D$ are known both to the defender and the attacker.\label{item_ass1}
    \item The defender cannot directly measure the attack $a$.\label{item_ass2}
    \item The defender can select the topology for all $t$ and the attacker knows the initial topology.\label{item_ass3}
    \item If the topology is switched at $t$, the attacker can detect it at $t+\Delta t_\nu$.\label{item_ass4}
    \item The actuation and sensing are performed discretely with the zero-order hold (\eg{},~\cite{zoh}), with $\Delta t_u$, $\Delta t_a$, $\Delta t_y$ being the control actuation, attack actuation, and sensing sampling period, respectively.\label{item_ass5}
    \item The topology $\nu(t)$ is fixed during $t\in[k\Delta t_y,(k+1)\Delta t_y],~\forall k \in \mathbb{N}$ with $\Delta t_y < \Delta t_{\nu}$.\label{item_ass6}
\end{enumerate}
\end{assumption}
Note that~\ref{item_ass5} of Assumption~\ref{assump_system} is just for representing one of the most practical and frequently used ways to perform actuation and sensing in modern control systems.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Zero Dynamics Attack}
\label{sec_zda_definitions}
The zero dynamics attack (ZDA) is a stealthy attack designed based on the assumptions \ref{item_ass1} and \ref{item_ass2} of Assumption~\ref{assump_system}. In this paper, we define a stealthy (or undetectable~\cite{attack_bullo}) attack and $\alpha$-stealthy as follows.
%%%
\begin{definition}
\label{def_stealth}
For a given terminal time $t_f$, an attack $a(t)$ of~\eqref{eq_continuous_initialx} is stealthy in $t\in[0,t_f]$ if, for some initial states, we have $y(t) = y_n(t)$ for $\forall t\in[0,t_f]$, where $y$ is given by~\eqref{eq_continuous_initialy} and $y_n$ is by $y$ of~\eqref{eq_continuous_initialy} with $a=0$.
\end{definition}
%%%
%\begin{definition}
%\label{def_alpha_stealth}
%For a given terminal time $t_f$, an attack $a(t)$ of~\eqref{eq_continuous_initialx} is $\alpha$-stealthy in $t\in[0,t_f]$ if, %for some initial states and $\alpha\in\mathbb{R}_{+}$, we have $\|y(t)-y_n(t)\|^2 \leq \alpha$ for $\forall t\in[0,t_f]$, where $y$ is given by~\eqref{eq_continuous_initialy} and $y_n$ is by $y$ of~\eqref{eq_continuous_initialy} with $a=0$.
%\end{definition}
%%%
This paper focuses on the ZDA as one of the most notorious but common stealthy attacks. It works for a wide range of real-world systems (\eg{}, robotics, aerospace, and cyber-physical systems) \textit{even when they are both controllable and observable}.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsubsection{Intrinsic ZDA}
This is a stealthy attack based on the invariant zeros $z_{\text{inv}} \in \mathbb{C}$ of the system~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy}, at which the following equation with the Rosenbrock system matrix
\begin{align}
    \label{eq_rosenbrock_cp}
    \begin{bmatrix}
    z_{\text{inv}}\mathbb{I}-A & -B_a \\
    C & D
\end{bmatrix}
\begin{bmatrix}
    x_{a0} \\ u_{a0}
\end{bmatrix} = 0
\end{align}
gives a nontrivial solution $[x_{a0}^{\top}~u_{a0}^{\top}]^{\top} \neq 0$, assuming that the topology $\nu$ is fixed. The intrinsic ZDA has a tight connection to the zero dynamics/internal dynamics of~\cite{zero_dynamics_isidori} that often appear in hybrid robotics~\cite{hybrid_robotics}. In fact, for linear systems, the system eigenvalues of the internal dynamics are equal to the invariant zeros of~\eqref{eq_rosenbrock_cp}~\cite[pp. 297-299]{Isidori:1995:NCS:545735}.
\begin{lemma}
\label{lemma_c_ZDA}
If there exist $z_{\text{inv}}$, $x_{a0}$, $u_{a0}$ that satisfy~\eqref{eq_rosenbrock_cp} and the topology is fixed, an attack constructed as $a = e^{z_{\text{inv}} t}u_{a0}$ with $x(0) = x_{n0}+x_{a0}$ is stealthy in the sense of Definition~\ref{def_stealth}, where $x_{n0}$ is a nominal initial state for~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy} with $a=0$.
\end{lemma}
\begin{proof}
Let $X(s) = \mathcal{L}[x(t)]$, $U(s) = \mathcal{L}[u(t)]$, and $Y(s) = \mathcal{L}[y(t)]$ for the Laplace transform $\mathcal{L}$. Since we have
\begin{align}
    &(s-z_{\text{inv}})^{-1}(z_{\text{inv}}\mathbb{I}-A) = -\mathbb{I}+(s-z_{\text{inv}})^{-1}(s\mathbb{I}-A)
\end{align}
for any $s$, applying $\mathcal{L}$ to~\eqref{eq_continuous_initialx} with the first row of~\eqref{eq_continuous_initialx} yields
\begin{align}
    X(s) = (s\mathbb{I}-A)^{-1}(x_{n0}+BU(s))+(s-z_{\text{inv}})^{-1}x_{a0}.
\end{align}
The second row of~\eqref{eq_rosenbrock_cp} with~\eqref{eq_continuous_initialy} then gives $Y(s)= C(s\mathbb{I}-A)^{-1}(x_{n0}+BU(s))+DU(s)$ as desired.
\end{proof}

Lemma~\ref{lemma_c_ZDA} indicates that the intrinsic ZDA stealthily makes $x$ of~\eqref{eq_continuous_initialx} diverge if the system is non-minimum-phase $\Leftrightarrow \operatorname{Re}(z_{\text{inv}}) > 0 \Leftrightarrow$ the internal dynamics is unstable (see~\cite{zda_discrete,zda_discrete2} for discrete-time systems and \cite{attack_bullo,zda_continuous_hovakimyan} for continuous-time systems for more details). The zeros $z_{\text{inv}}$ are ``invariant'' under coordinate changes and state feedback, which represent one of the ``intrinsic'' properties of internal dynamics.
%%%
%%%
\begin{example}
\label{ex_cp}
The linearized dynamical system of the cart-pole balancing with the position measurement is subject to the ZDA although it is both controllable and observable. This is part of the reason why the ZDA can be a great threat in robotics~\cite{hybrid_robotics} (see Fig.~\ref{fig_ex_cp_attack}). Some other examples include, but are not limited to, the PVTOL aircraft~\cite{pvtol}, bipedal/quadrupedal robots~\cite{hybrid_robotics}, UAVs~\cite{uavzda}, and robotic manipulators~\cite{nmpzeros}.
%%%
\begin{figure}
    \centering
    \includegraphics[height=24mm]{figures/examples/ex_cp_stacked.pdf}
    \caption{Cart-pole balancing with the intrinsic ZDA, where $x$ is the cart's position, $v$ is the velocity, $\phi$ is the pole's angle from the upward equilibrium, and $\omega$ is the angular velocity as described \textcolor{uiucblue}{\href{https://ctms.engin.umich.edu/CTMS/index.php?example=InvertedPendulum&section=SystemModeling}{here}}. Due to the stealthy nature of the ZDA, the states estimated by the Kalman filter erroneously converge although the actual states diverge.}
    \label{fig_ex_cp_attack}
\end{figure}
%%%
\end{example}
%%%
%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsubsection{Sampling ZDA}
Discretization of~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy} could introduce additional potentially unstable zeros, called sampling zeros~\cite{zoh}. In fact, if the system's relative degree is $\geq 3$, we always have at least one unstable sampling zero~\cite[pp. 47-58]{yuz_sampled-data_2014} in addition to the intrinsic invariant zeros.

The sampling ZDA, introduced in~\cite{sampling_zda}, essentially uses these zeros in the discretized system of~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy}, which can be computed as in~\eqref{eq_rosenbrock_cp} by replacing its system matrices with the discretized counterparts. 
\begin{lemma}
\label{lemma_d_ZDA}
If there exist $z_{\text{inv}}$, $x_{a0}$, $u_{a0}$ that satisfy~\eqref{eq_rosenbrock_cp} for the discretized system and the topology is fixed, an attack constructed as $a = z_{\text{inv}}^ku_{a0}$ with $x(0) = x_{n0}+x_{a0}$ is stealthy in the sense of Definition~\ref{def_stealth}, where $x_{n0}$ is a nominal initial state for~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy} with $a=0$.
\end{lemma}
\begin{proof}
This follows from taking the Z-transform instead of the Laplace transform for the discretized system in Lemma~\ref{lemma_c_ZDA}.
\end{proof}
It can be computed as $a_i = z_{\text{inv}}^iu_{a0}$ with the time step index $i$ (\cite[p. 88]{robust_control_book_doyle} with the Z-transform), which indicates that it stealthily makes $x$ of~\eqref{eq_continuous_initialx} diverge if the discretized system is non-minimum-phase $\Leftrightarrow |z_{\text{inv}}| > 1 \Leftrightarrow$ the discretized internal dynamics is unstable. Some examples, including connected double integrators with feedback communications, are given in~\cite{zda_tutorial} and the references therein.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsubsection{Enforced ZDA}
Even if the discretized system is minimum-phase (\ie, there are no unstable zeros), the attacker can still easily design a disruptive stealthy attack by exploiting actuation redundancy/asynchronous actuation and sensing of~\ref{item_ass5} in Assumption~\ref{assump_system}. Such an attack is called the enforced ZDA~\cite{enforced_zda, zda_tutorial}. This significantly broadens the applicability of ZDAs to controllable, observable, and minimum-phase real-world systems with discrete-time actuation and sensing.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Motivation and Problem Statement}
As implied in Sec.~\ref{sec_zda_definitions}, the only possible way for detecting ZDAs is to change the underlying dynamical system somehow in~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy}, which motivates us to consider optimal and robust topology switching.
%%%
%%%
\begin{example}
\label{ex_dinet}
Let us consider the network of six 3D double integrators with the enforced ZDA to see the effectiveness of topology switching. We consider the two topologies given on the right-hand side of Fig.~\ref{fig_ex_dinet_attack}, both of which are controllable, observable, and minimum-phase with the full position measurements, where we simply assume a position feedback synchronization controller. As can be seen on the left-hand side of Fig.~\ref{fig_ex_dinet_attack}, the enforced ZDA is indeed completely stealthy initially but switching the topology makes the attack visible in the measurement.
%%%
\begin{figure}
    \centering
    \includegraphics[height=24mm]{figures/examples/ex_dinet_stacked.pdf}
    \caption{Networks of 3D double integrators with the enforced ZDA. Although the attack is stealthy initially, the topology switching reveals it at $t = 50$ (sec).}
    \label{fig_ex_dinet_attack}
\end{figure}
%%%
\end{example}
%%%
%%%

How can we formalize such topology switching so the defender can optimally and robustly detect the disruptive ZDAs of Sec.~\ref{sec_zda_definitions}?
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%

==> sections/archived_sections/4_metrics.tex <==
\section{Performance Metrics for Topology Switching}
\label{sec_metrics}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
In order to quantify the quality of the topology switching demonstrated in Example~\ref{ex_dinet}, this section defines several performance metrics expressed explicitly in terms of the network topology $\nu$ of~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy}. We especially focus on finite-horizon metrics so we can handle time-varying defense and detection strategies.
\begin{remark}
\label{ref_remnote}
In the subsequent discussion, we suppose that Assumption~\ref{assump_system} holds unless stated otherwise. Also, we let $i$, $j$, and $k$ be the sampling indices for the control, attack, and sensing, respectively, $t_f$ be the terminal time, $x_S$ is the initial state, $x_F$ is the terminal state, $t_i = i\Delta t_u$, $t_j = j\Delta t_a$, $t_k = k\Delta t_y$ for the time periods of~\ref{item_ass5}, $I = \floor{t_f/\Delta t_u}$, $J = \floor{t_f/\Delta t_a}$, $K = \floor{t_f/\Delta t_y}$ for the floor function $\floor{\cdot}$, and $u_i = u(t_i)$, $a_j = a(t_j)$, $x_k = x(t_k)$, $A_k = e^{A(\nu(t_k))\Delta t_y}$, $B_{u,k} = B_u(\nu(t_k))$, $B_{a,k} = B_a(\nu(t_k))$, $C_k = C(\nu(t_k))$, and $D_k = D(\nu(t_k))$ in the system~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy}.
\end{remark}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Discretization with Asynchronous Actuation and Sensing}
Before we proceed, let us compute the discretized counterparts of~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy} with the asynchronous actuation and sensing of Assumption~\ref{assump_system}. This is achieved simply by using the impulse response $h_{\mu}(t)$ of the zero-order hold, given as $h_{\mu}(t) = 1$ if $t \in [0,\Delta t_{\mu})$ \& $h_{\mu}(t) = 0$ otherwise, which results in the control and attack input expressed as 
\begin{align}
    \label{eq_mu_def}
    \mu(t) = \sum_{\ell=0}^{\Ell}h_{\mu}(t-t_\ell)u_\ell
\end{align}
where $(\mu,\ell,\Ell)\in\{(u,I,I),(a,j,J)\}$.
%%%%%
%%%%%
%%%%%
\begin{lemma}
\label{lemma_discretization}
Let us use the notation in Remark~\ref{ref_remnote} and define $\mathbf{B}_{\mu,k,\Ell}$ as
\begin{align}
    \mathbf{B}_{\mu,k,\Ell} =
    \begin{bmatrix}
        H_{\mu,k,0}B_{\mu,k} & H_{\mu,k,1}B_{\mu,k} & \cdots & H_{\mu,k,\Ell}B_{\mu,k}
    \end{bmatrix}
\end{align}
for $(\mu,\ell,\Ell)\in\{(u,I,I),(a,j,J)\}$ and 
\begin{align}
    \label{eq_Himpulsedef}
    H_{\mu,k,\ell} = \int_{t_k}^{t_{k+1}}e^{A_k(t_{k+1}-\tau)}h_\mu(\tau-t_\ell)d\tau.
\end{align}
If \ref{item_ass5}~and~\ref{item_ass6} of Assumption~\eqref{assump_system} hold, the dynamics~\eqref{eq_continuous_initialx} is discretized as follows:
\begin{align}
    \label{eq_all_state}
    \mathbf{x}_{K} &= \mathcal{A}_{K}x_S+\mathcal{B}_{u,K,I}\mathbf{u}_{I}+\mathcal{B}_{a,K,J}\mathbf{a}_{J}
\end{align}
where $\mathcal{A}_{K} = [\mathbb{I}^{\top},A_0^{\top},(A_1A_0)^{\top},\cdots,(A_{K-1}\cdots A_0)^{\top}]^{\top}$, $\mathbf{x}_K = [x_0^{\top},\cdots,x_K^{\top}]^{\top}$, $\mathbf{u}_I = [u_0^{\top},\cdots,u_{I}^{\top}]^{\top}$, $\mathbf{a}_{J} = [a_{0}^{\top},\cdots,a_{J}^{\top}]^{\top}$, and
\begin{align}
    \mathcal{B}_{\mu,K,\Ell} = 
    \begin{bmatrix}
        \mathbb{O} \\
        \mathbf{B}_{\mu,0,L} \\
        A_1\mathbf{B}_{\mu,0,L}+\mathbf{B}_{\mu,1,L} \\
        \vdots \\
        A_{K-1}\cdots A_1\mathbf{B}_{\mu,0,L}+\cdots+\mathbf{B}_{\mu,K-1,L}
    \end{bmatrix}.~\label{eq_Bmathcaldef}
\end{align}
Also, using the block diagonal matrix $\blkdiag{(\cdot)}$, the measurement~\eqref{eq_continuous_initialy} can be computed as follows:
\begin{align}
    \label{eq_all_measurement}
    \mathbf{y}_K = \mathcal{C}_K\mathcal{A}_{K}x_S+\mathcal{C}_K\mathcal{B}_{u,K,I}\mathbf{u}_{I}+(\mathcal{C}_K\mathcal{B}_{a,K,J}+\mathcal{D}_K\mathcal{H}_{a,K,J})\mathbf{a}_{J}~~~~~
\end{align}
where $\mathcal{C}_K = \blkdiag{(C_0,\cdots,C_K)}$, $\mathcal{D}_K = \blkdiag{(D_0,\cdots,D_K)}$, $\mathbf{y}_K = [y_0^{\top},\cdots,y_{K-1}^{\top},y_K^{\top}]^{\top}$, and
\begin{align}
    \mathcal{H}_{a,K,J} =
    \begin{bmatrix}
    h_a(t_0-t_0) & \cdots & h_a(t_0-t_J) \\
    \vdots & \ddots & \vdots \\
    h_a(t_K-t_0) & \cdots & h_a(t_K-t_J)
    \end{bmatrix}.
\end{align}
\end{lemma}
\begin{proof}
Integrating~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy} with $u(t)$ and $a(t)$ given by~\eqref{eq_mu_def} completes the proof.
\end{proof}
%%%%%
%%%%%
%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Transient Controllability Metric}
The minimum control effort to reach the terminal state $x_F$ from the initial state, which characterizes the system's controllability, can be computed as follows assuming $\mathbf{a}_{J} = 0$ in~\eqref{eq_all_state}~\cite{gramian_original}:
\begin{align}
    \label{eq_controllability_obj}
    &\bar{J}_{\text{con}}(\nu,x_S,x_F) = \inf_{\mathbf{u}_I}\mathbf{u}_I^{\top}\mathbf{Q}_{\text{con}}^{-1}\mathbf{u}_I \\
    &\text{\st{}}~\mathbf{x}_{K} = \mathcal{A}_{K}x_S+\mathcal{B}_{u,K,I}\mathbf{u}_{I},~x_K=x_F \label{eq_controllability_con}
\end{align}
where the notation is consistent with~\eqref{eq_all_state} and $\mathbf{Q}_{\text{con}}\succ0$ is the weight on the control input.
%%%%%
%%%%%
%%%%%
\begin{lemma}
\label{lemma_controllability}
If $(\mathcal{B}_{u,K,I})_K\mathbf{Q}_{\text{con}}^{-1}(\mathcal{B}_{u,K,I})_K^{\top}$ is invertible, the metric of~\eqref{eq_controllability_obj} is given as
\begin{align}
    \label{eq_controllability_explicit}
    \bar{J}_{\text{con}} = \Delta x_{SF}^{\top}\left((\mathcal{B}_{u,K,I})_K\mathbf{Q}_{\text{con}}(\mathcal{B}_{u,K,I})_K^{\top}\right)^{-1}\Delta x_{SF}
\end{align}
where $\Delta x_{SF} = x_F-(\mathcal{A}_K)_Kx_S$, $(\mathcal{A}_K)_K$ and $(\mathcal{B}_{u,K,I})_K$ are the last $n$ rows of $\mathcal{A}_K$ and $\mathcal{B}_{u,K,I}$, respectively, and the other notations are given in~\eqref{eq_all_state} and in Remark~\ref{ref_remnote}.
\end{lemma}
\begin{proof}
Since the problem~\eqref{eq_controllability_obj} is convex, applying the KKT condition completes the proof.
\end{proof}
%%%%%
%%%%%
%%%%%

We thus define the following transient controllability metric as a result of Lemma~\ref{lemma_controllability}:
\begin{align}
    \label{eq_controllability_explicit_final}
    J_{\text{con}}(\nu) = \lambda_{\min}\left((\mathcal{B}_{u,K,I})_K\mathbf{Q}_{\text{con}}(\mathcal{B}_{u,K,I})_K^{\top}\right)
\end{align}
where $\lambda_{\min}(\cdot)$ denotes the minimum eigenvalue.
\begin{remark}
When the actuation and sensing frequencies are equal (\ie{}, $\Delta t_u = \Delta t_y$), the term $(\mathcal{B}_{u,K,I})_K\mathbf{Q}_{\text{con}}(\mathcal{B}_{u,K,I})_K^{\top}$ in~\eqref{eq_controllability_explicit_final} reduces to the (weighted) controllability Gramian~\cite{gramian_original} and can be computed recursively.
\end{remark}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Transient Observability Metric}
Similarly, given an initial state $x_S$, this metric can be characterized as follows assuming $\mathbf{u}_{I} = \mathbf{a}_{J} = 0$ in~\eqref{eq_all_measurement}~\cite{gramian_original}:
\begin{align}
    \bar{J}_{\text{obs}}(\nu,x_S) &= \mathbf{y}_K^{\top}\mathbf{Q}_{\text{obs}}\mathbf{y}_K~\text{\st{}}~\mathbf{y}_K = \mathcal{C}_K\mathcal{A}_{K}x_S \\
    &= \mathbf{y}_K^{\top}\mathcal{A}_{K}^{\top}\mathcal{C}_K^{\top}\mathbf{Q}_{\text{obs}}\mathcal{C}_K\mathcal{A}_{K}\mathbf{y}_K
    \label{eq_observability_explicit}
\end{align}
where the notation is consistent with~\eqref{eq_all_measurement} and $\mathbf{Q}_{\text{obs}}\succ0$ is the weight on the measurement. Since observability is not affected by the asynchronous nature discussed in Lemma~\ref{lemma_discretization}, we have the (weighted) observability Gramian $\mathcal{A}_{K}^{\top}\mathcal{C}_K^{\top}\mathbf{Q}_{\text{obs}}\mathcal{C}_K\mathcal{A}_{K}$ in~\eqref{eq_observability_explicit} as expected.

We thus define the following transient observability metric:
\begin{align}
    \label{eq_observability_explicit_final}
    J_{\text{obs}}(\nu) = \lambda_{\min}\left(\mathcal{A}_{K}^{\top}\mathcal{C}_K^{\top}\mathbf{Q}_{\text{obs}}\mathcal{C}_K\mathcal{A}_{K}\right)
\end{align}
where $\lambda_{\min}(\cdot)$ denotes the minimum eigenvalue.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Transient Attack Robustness Metric}
The metric can be defined with the following transient $\mathcal{H}_{\infty}$ norm (or $\mathcal{L}_2$ gain in a nonlinear sense)~\cite[Sec.~5.3]{Khalil:1173048} from the attack $\mathbf{a}_J$ and the initial state $x_S$ to the full state $\mathbf{x}_K$, assuming $\mathbf{u}_I = 0$ in~\eqref{eq_all_state}:
\begin{align}
    &J_{\text{rob}}(\nu) = \sup_{x_S,\mathbf{a}_J}\mathbf{x}_K^{\top}\mathbf{Q}_{\text{rob}}\mathbf{x}_K \label{eq_robustness_obj} \\
    &\text{\st{}}~\mathbf{x}_{K} = \mathcal{A}_{K}x_S+\mathcal{B}_{a,K,J}\mathbf{a}_{J},~\|x_S\|^2+\|\mathbf{a}_J\|^2 \leq 1 \label{eq_robustness_con}
\end{align}
where the notation is consistent with~\eqref{eq_all_state}, $\mathbf{Q}_{\text{rob}}\succ0$ is the weight on the state, and $\|x_S\|^2+\|\mathbf{a}_J\|^2 \leq 1$ is introduced here to avoid the trivial solution of $\mathbf{a}_J = \infty$ as in the operator norm.
%%%%%
%%%%%
%%%%%
\begin{lemma}
\label{lemma_robustness}
The attack robustness metric of~\eqref{eq_robustness_obj} is given as
\begin{align}
    \label{eq_robust_explicit}
    J_{\text{rob}}(\nu) = \lambda_{\max}\left(
    \begin{bmatrix}
        \mathcal{A}_{K}^{\top} \\ \mathcal{B}_{a,K,J}^{\top}
    \end{bmatrix}
    \mathbf{Q}_{\text{rob}}
    \begin{bmatrix}
        \mathcal{A}_{K} & \mathcal{B}_{a,K,J}
    \end{bmatrix}\right)
\end{align}
where $\lambda_{\max}(\cdot)$ denotes the maximum eigenvalue and the other notations are given in~\eqref{eq_all_state} and in Remark~\ref{ref_remnote}.
\end{lemma}
\begin{proof}
Using the first constraint of~\eqref{eq_robustness_con}, we get $\mathbf{x}_K^{\top}\mathbf{Q}_{\text{rob}}\mathbf{x}_K = [x_S^{\top},\mathbf{a}_{J}^{\top}][\mathcal{A}_{K},\mathcal{B}_{a,K,J}]^{\top}\mathbf{Q}_{\text{rob}}[\mathcal{A}_{K},\mathcal{B}_{a,K,J}][x_S^{\top},\mathbf{a}_{J}^{\top}]^\top$. Since $[\mathcal{A}_{K},\mathcal{B}_{a,K,J}]^{\top}\mathbf{Q}_{\text{rob}}[\mathcal{A}_{K},\mathcal{B}_{a,K,J}]\succeq 0$, upper-bounding this relation using the second constraint of~\eqref{eq_robustness_con} yields~\eqref{eq_robust_explicit}. The fact that the bound is the supremum can be shown by contradiction~\cite[p. 210]{Khalil:1173048}
\end{proof}
%%%%%
%%%%%
%%%%%
\begin{remark}
Although we consider the controllability and attack robustness separately to access each property individually, we could also combine them to get what is called the game-theoretic controllability Gramian~\cite{Basar1995,learning_actuator_selection}.
\end{remark}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Transient Minimum Attack Sensitivity Metric}
This is the most important metric for the detection of the ZDAs introduced in~\eqref{sec_zda_definitions}, which measures the stealthiness of malicious attacks. Given an initial state $x_S$, this metric can be defined with the following transient $\mathcal{H}_{-}$ index~\cite{security_metric_book,Hsubobserver,LMIsensitivity,secure_control,outputL2gain}, assuming $\mathbf{u}_I = 0$ in~\eqref{eq_all_measurement}:
\begin{align}
    &J_{\text{sen}}(\nu) = \inf_{x_S,\mathbf{a}_J}\mathbf{y}_K^{\top}\mathbf{Q}_{\text{sen}}\mathbf{y}_K \label{eq_sensitivity_obj} \\
    &\text{\st{}}~
    \mathbf{y}_K = \mathcal{C}_K\mathcal{A}_{K}x_S+(\mathcal{C}_K\mathcal{B}_{a,K,J}+\mathcal{D}_K\mathcal{H}_{a,K,J})\mathbf{a}_{J}\label{eq_sensitivity_con1} \\
    &{\textcolor{white}{\text{\st{}}}}~\|x_S\|^2+\|\mathbf{a}_J\|^2 \geq 1\label{eq_sensitivity_con2}
\end{align}
where the notation is consistent with~\eqref{eq_all_measurement}, $\mathbf{Q}_{\text{sen}}\succ0$ is the weight on the measurement, and $\|x_S\|^2+\|\mathbf{a}_J\|^2 \geq 1$ is introduced here to avoid the trivial solution of $x_S = 0$ and $\mathbf{a}_J = 0$ as in the ZDA~\eqref{eq_rosenbrock_cp}.
%%%%%
%%%%%
%%%%%
\begin{lemma}
\label{lemma_sensitivity}
The minimum attack sensitivity metric of~\eqref{eq_sensitivity_obj} is given as
\begin{align}
    \label{eq_sensitivity_explicit}
    J_{\text{sen}}(\nu) = \lambda_{\min}\left(
    \begin{bmatrix}
        \mathcal{A}_{K}^{\top}\mathcal{C}_K^{\top} \\ \mathcal{E}_{a,K,J}^{\top}
    \end{bmatrix}
    \mathbf{Q}_{\text{sen}}
    \begin{bmatrix}
        \mathcal{C}_K\mathcal{A}_{K} & \mathcal{E}_{a,K,J}
    \end{bmatrix}\right)
\end{align}
where $\mathcal{E}_{a,K,J} = \mathcal{C}_K\mathcal{B}_{a,K,J}+\mathcal{D}_K\mathcal{H}_{a,K,J}$, $\lambda_{\min}(\cdot)$ denotes the minimum eigenvalue, the other notations are given in~\eqref{eq_all_measurement} and in Remark~\ref{ref_remnote}.
\end{lemma}
\begin{proof}
The result~\eqref{eq_sensitivity_explicit} follows from lower-bounding the posotive semi-definite matrix $\mathbf{y}_K^{\top}\mathbf{Q}_{\text{sen}}\mathbf{y}_K$ using~\eqref{eq_sensitivity_con1}~and~\eqref{eq_sensitivity_con2} as in the proof of Lemma~\ref{lemma_robustness}.
\end{proof}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\if0
\subsection{Transient Stealthy Attack Robustness Metric}
Inspired by the $\mathcal{H}_{\infty}$ norm (or $\mathcal{L}_2$ gain in a nonlinear sense)~\cite[Sec.~5.3]{Khalil:1173048}, this metric measures the robustness of the system Flemma
from the attack $\mathbf{a}_J$ and the initial state $x_S$ to the full state $\mathbf{x}_K$, assuming $\mathbf{u}_I = 0$ in~\eqref{eq_all_state}:

This is the most important metric for the detection of the ZDAs introduced in~\eqref{sec_zda_definitions}, which measures the stealthiness of malicious attacks. Given an initial state $x_S$, this metric can be defined with the following transient $\mathcal{H}_{-}$ index~\cite{security_metric_book,Hsubobserver,LMIsensitivity,secure_control,outputL2gain}, assuming $\mathbf{u}_I = 0$ in~\eqref{eq_all_measurement}:

This metric provides 
The minimum attack sensitivity metric of~\eqref{eq_sensitivity_obj} is given as
\begin{align}
    \label{eq_sensitivity_explicit}
    J_{\text{sen}}(\nu) = \lambda_{\min}\left(
    \begin{bmatrix}
        \mathcal{A}_{K}^{\top}\mathcal{C}_K^{\top} \\ \mathcal{E}_{a,K,J}^{\top}
    \end{bmatrix}
    \mathbf{Q}_{\text{sen}}
    \begin{bmatrix}
        \mathcal{C}_K\mathcal{A}_{K} & \mathcal{E}_{a,K,J}
    \end{bmatrix}\right)
\end{align}
\TBD{combine the robustness and sensitivity using the output-to-output L2 gain}
\fi
%%%%%
%%%%%
%%%%%

==> sections/archived_sections/5_switching.tex <==
\section{Robust Optimal Topology Switching}
\label{sec_switching}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
Now that we have some metrics for quantifying the performance of the system~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy}, this section presents several numerically efficient optimization approaches for designing switching strategies of the network topology. We still suppose that Assumption~\ref{assump_system} holds and we use the notation of Remark~\ref{ref_remnote}.
\begin{itemize}
    \item \textcolor{caltechred}{Prove that output-to-output feedback -> dual problem Hinfinity like formulation and prove zero duality gap...}
    \item \textcolor{caltechred}{Stealthiness is not affected by feedback}
\end{itemize}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Topology Feedback Control}
Feedbacking the network state as follows provides additional control authority over the modification of the system matrices:
\begin{align}
    \label{eq_feedback_control}
    \mathbf{u}_I &=  \mathcal{K}_{K,I}\mathbf{x}_K+\Lambda_{a}\mathbf{a}_J+\mathbf{v}_I \\
    &= 
    \begin{bmatrix}
    f_{s}(t_0-t_0)K_{0,0} & \cdots & f_{s}(t_0-t_K)K_{0,K} \\
    \vdots & \ddots & \vdots \\
    f_{s}(t_I-t_0)K_{I,0} & \cdots & f_{s}(t_I-t_K)K_{I,K}
    \end{bmatrix}\mathbf{x}_K+\Lambda_{a}\mathbf{a}_J+\mathbf{v}_I
\end{align}
where $\mathbf{x}_K$ and $\mathbf{u}_I$ are as given in Lemma~\ref{lemma_discretization}, $\mathbf{v}_I$ is a residual control input for additional tasks, $K_{i,k} \in \mathbb{R}^{q\times p}$ are the control gains, $\Lambda_{a}\mathbf{a}_J$ represents the adversarial feedback due to the sensor attack with $\Lambda_{a} \in \mathbb{R}^{qI\times rJ}$, and $f_{s}$ is the unit step function, \ie{}, $f_{s}(t) = 1$ if $t\geq 0$ and $f_{s}(t) = 0$ otherwise. The step functions are just for ensuring the causality of the state feedback.
\begin{remark}
The formulation of~\eqref{eq_feedback_control} does not mean that the system has access to the full state. In fact, if we have feedback only on the system output, we can simply modify $\mathcal{K}_{K,I}$ as $\mathcal{K}_{K,I} = \mathcal{K}\mathcal{C}_K$ and $\Lambda_{a}$ as $\Lambda_{a} = \Lambda\mathcal{D}_K$, where $\mathcal{K}$ and $\Lambda$ are some constants. Also, if we view the state $\mathbf{x}_K$ as the augmented state of the actual state $\mathbf{x}_{\text{act}}$ and the estimated state $\mathbf{x}_{\text{est}}$, \ie{}, $\mathbf{x}_K = [\mathbf{x}_{\text{act}}^{\top},\mathbf{x}_{\text{est}}^{\top}]^{\top}$, as discussed in Remark~\ref{remark_estimation}, we can select $K_{i,k}$ to have $\mathcal{K}_{K,I}\mathbf{x}_K = [\mathbb{O},\mathcal{K}_{\text{est},K,I}]\mathbf{x}_K$ to express output feedback, where $\mathcal{K}_{\text{est},K,I}$ is the feedback gain for the estimated state. See~\cite{outputL2gain} for more details.
\end{remark}

Using the feedback control policy~\eqref{eq_feedback_control} in~\eqref{eq_all_state}, we have
\begin{align}
    \label{eq_control_substitute}
    \mathcal{L}_{K,I}\mathbf{x}_{K} &= \mathcal{A}_{K}x_S+\mathcal{B}_{u,K,I}\mathbf{v}_I+(\mathcal{B}_{a,K,J}+\mathcal{B}_{u,K,I}\Lambda_a)\mathbf{a}_{J}. \\
    \mathcal{L}_{K,I} &= \mathbb{I}-\mathcal{B}_{u,K,I}\mathcal{K}_{K,I}
    \label{eq_control_gain_L}
\end{align}
The following lemma derives an explicit form of $\mathbf{x}_{K}$ under the feedback control.
\begin{lemma}
The matrix $\mathcal{L}_{K,I}$ of~\eqref{eq_control_gain_L} is invertible and thus we have the following:
\begin{align}
    \label{eq_control_state_explicit}
    \mathbf{x}_{K} &= \mathcal{L}_{K,I}^{-1}(\mathcal{A}_{K}x_S+\mathcal{B}_{u,K,I}\mathbf{v}_I+\mathcal{B}_{a,K,J}\mathbf{a}_{J}).
\end{align}
\end{lemma}
\begin{proof}
By definition of $H_{u,k,i}$ in~\eqref{eq_Himpulsedef} and the step function $f_{s}$ in~\eqref{eq_feedback_control}, we have
\begin{align}
    H_{u,k,i}f_{s}(t_i-t_{l})K_{i,l} = 0 & \text{ if $k+1 \leq l$}.
\end{align}
This indicates that the matrix $\mathcal{B}_{u,K,I}\mathcal{K}_{K,I}$ is strictly lower triangular for $\mathcal{B}_{u,K,I}$ of~\eqref{eq_Bmathcaldef}, which can be shown also by the system's causality. The rest follows from~\eqref{eq_control_substitute}.
\end{proof}

In the subsequent discussion, we consider the entries of the weighted adjacency matrix of the network, denoted by $\Theta \in \mathbb{R}_{+}^{N\times N}$, as the parameter for beginning the network topology $\nu$ of~\eqref{eq_continuous_initialx}~and~\eqref{eq_continuous_initialy}, where $\mathbb{R}_{+}^{N\times N}$ is the set of $N$ by $N$ matrices with non-negative entries and $N$ is the number of agents. We assume the following.
\begin{assumption}
The discretized system matrices $A_{k}$, $B_{u,k}$, $B_{a,k}$, $C_{k}$, and $D_{k}$ of Lemma~\ref{lemma_discretization}, and the control gains $K_{i,k}$ and $\Lambda_{a}$ of~\eqref{eq_feedback_control} relate affinely to the parameter $\Theta$ of the network topology $\nu$. 
\end{assumption}
\TBD{Note that we do not assume that the network is balanced or strongly connected~\cite{Ref:phasesync}.}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Topology Switching with Fixed $A$}
In most of the practical networked control systems in robotics, aerospace, and cyber-physical systems, the system matrix $A$ of the system~\eqref{eq_continuous_initialx} is determined by the underlying physics and is not a function of the topology $\nu$. We thus start our discussion focusing on the case with $\partial A(\nu)/\partial \nu = 0$ in~\eqref{eq_continuous_initialx}

\textcolor{red}{The best we can achieve right now
\begin{itemize}
    \item Suppose sensor topology and actuation topology are different in terms of weights, which I think is possible
    \item Suppose that $D_a = 0$ (\sout{maybe not? because observability is invariant under feedback}, this is required because then we have inverse of $\mathcal{K}$ in $J_{\text{sen}}$)
    \item Suppose that and $\mathcal{A}$ and $\mathcal{B}$ are constants (maybe $\mathcal{B}$ could depend on $\nu$..)
    \item Then we may be able to show that the problem is BMI optimization?
    \item If we drop the observability condition, then the problem may still be BMI optimization
\end{itemize}
}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsubsection{Constraints and Objective}
Controllability, observability, and non-stealthiness (given in Difinition~\ref{def_stealth}) can be guaranteed as long as the controllability, observability, and minimum attack sensitivity metrics are positive, respectively, and thus they are best used as constraints. Also, it is well-known that controllability and observability are invariant under state feedback. Similarly, non-stealthiness can be shown to be invariant under state feedback as follows.
\begin{lemma}
\label{lemma_nonstealthy}
If $a$ Feedback control defined as in~\eqref{eq_feedback_control} does not change stealthiness if , \ie{}, if $\exists \mathcal{K}_{K,I}$ \st{} $J_{\text{sen}}(\nu) > 0$, then $J_{\text{sen}}(\nu) > 0,~\forall \mathcal{K}_{K,I}$, and if $\exists \mathcal{K}_{K,I}$ \st{} $J_{\text{sen}}(\nu) = 0$, then $J_{\text{sen}}(\nu) = 0,~\forall \mathcal{K}_{K,I}$.
\end{lemma}


As a result of Lemma
Let us consider the following optimization problem for topology switching:
\begin{align}
    &\min_{\Theta \in \mathbb{R}_{+}^{N\times N}}J_{\text{rob}}(\nu(\Theta)) = \lambda_{\max}\left(
    \begin{bmatrix}
        \mathcal{A}_{K}^{\top} \\ \mathcal{B}_{a,K,J}^{\top}
    \end{bmatrix}
    \mathbf{Q}_{\text{rob}}
    \begin{bmatrix}
        \mathcal{A}_{K} & \mathcal{B}_{a,K,J}
    \end{bmatrix}\right) \\
    &\text{\st{} }J_{\text{sen}}(\nu(\Theta)) = \lambda_{\min}\left(
    \begin{bmatrix}
        \mathcal{A}_{K}^{\top}\mathcal{C}_K^{\top} \\ \mathcal{E}_{a,K,J}^{\top}
    \end{bmatrix}
    \mathbf{Q}_{\text{sen}}
    \begin{bmatrix}
        \mathcal{C}_K\mathcal{A}_{K} & \mathcal{E}_{a,K,J}
    \end{bmatrix}\right) \neq 0
\end{align}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Synchronization and Tracking Guarantees}
\begin{itemize}
    \item Use~\cite{Ref:phasesync} to prove synchronization with weekly connected and unbalanced graphs, assuming ZDA detected + observability
\end{itemize}
